Can We Edit Multimodal Large Language Models?

In this paper, we focus on editing Multimodal Large Language Models (MLLMs). Compared to editing single-modal LLMs, multimodal model editing is more challenging, which demands a higher level of scrutiny and careful consideration in the editing process. To facilitate research in this area, we construct a new benchmark, dubbed MMEdit, for editing multimodal LLMs and establishing a suite of innovative metrics for evaluation. We conduct comprehensive experiments involving various model editing baselines and analyze the impact of editing different components for multimodal LLMs. Empirically, we notice that previous baselines can implement editing multimodal LLMs to some extent, but the effect is still barely satisfactory, indicating the potential difficulty of this task. We hope that our work can provide the NLP community with insights. Code and dataset are available in https://github.com/zjunlp/EasyEdit.

==> table/main_result.tex <==
% \renewcommand{\arraystretch}{1}
% \newcommand\resulttablefontsize{\fontsize{7.7pt}{9.24pt}\selectfont}
% \newcommand{\first}{\colorbox{blue!25}}
% \newcommand{\second}{\colorbox{blue!10}}

\begin{table*}[t]
	\centering

	\resulttablefontsize
	%\scriptsize
	%\footnotesize
	\setlength{\tabcolsep}{4pt}
	%\hfill{}
         \resizebox{2\columnwidth}{!}{
	\begin{tabular}{l c c c c c | c c c c }

		%\toprule
	\toprule
	\multicolumn{2}{c}{} & \multicolumn{4}{c}{\textsc{Editing VQA}}  & \multicolumn{4}{c}{\textsc{Editing Image Caption}}  \\
	    \cmidrule(r){3-6}  \cmidrule(r){7-10} 
		& \multicolumn{1}{c}{Method} &  \multicolumn{1}{c}{Reliability}$\uparrow$  & \multicolumn{1}{c}{T-Generality}$\uparrow$  & \multicolumn{1}{c}{T-Locality }$\uparrow$ & \multicolumn{1}{c}{M-Locality}$\uparrow$ & \multicolumn{1}{c}{Reliability}$\uparrow$ & \multicolumn{1}{c}{T-Generality}$\uparrow$ & \multicolumn{1}{c}{T-Locality}$\uparrow$ & \multicolumn{1}{c}{M-Locality}$\uparrow$ \\
        \midrule
		\multicolumn{1}{l}{\scriptsize \textcolor{darkgray}{}} &\multicolumn{8}{c}{\textbf{\small BLIP-2 OPT}}  & \multicolumn{1}{r}{\scriptsize \textcolor{darkgray}{Size: 3.8B}} \\
		\midrule
		\multirow{3}{*}{Base Methods} & Base Model & 0.00 & 0.00 & 100.0 & 100.0 & 0.00 & 0.00 & 100.0 & 100.0    \\
		& FT (vision block) & 56.28 & 29.88 & 100.0 & 11.32 & 0.08 & 0.00 & 100.0 & 7.31  \\
		& FT (last layer) & 58.70 & 15.33 & 78.86 & 2.86 & 0.24 & 0.10 & 67.67 & 3.91 \\
            \midrule
		\multirow{4}{*}{Model Editing} & Knowledge Editor & 67.80 & 63.00 & \second{97.32} & \second{45.89} & 69.00 & 62.80 & \second{96.21} & \second{45.55}   \\
          & In-Context Editing & \first{99.95} & \first{91.59} & 13.16 & 1.88 & \first{96.70} & \second{78.20} & 13.36 & 2.17 \\
		% & MEMIT &  &  &  &  &  & \:\:\:  \\
	   & SERAC & 91.20 & \second{91.40} & \first{100.0} & 0.33 & \second{94.40} & \first{96.00} & \first{100.0} & 0.47  \\
          & MEND & \second{92.60} & 90.80 & 96.07 & \first{65.15} & 65.00 & 38.00 & 92.67 & \first{55.72} \\
		% \midrule
  %       %\arrayrulecolor{lightgray}\midrule\arrayrulecolor{black}
  %       \multirow{2}{*}{Input Augmentation} & Definition &{ 60.0 ($+$25.9)}  &\textit{ 34.1} & 22.5 ($-$16.3)  & \textit{ 26.1}  & \:\:\:\:3.2 ($-$17.9)  & \textit{26.1}  \\
  %       & Random Def. & 27.7 ($-$6.4)\:\:  &\textit{ 34.1} & 55.1 ($+$16.3)  & \textit{ 26.1}  &  \:\:35.7 ($+$14.6) &  \textit{26.1} \\
		\midrule
		\multicolumn{1}{l}{\scriptsize \textcolor{darkgray}{}} & \multicolumn{8}{c}{\textbf{\small MiniGPT-4}} & \multicolumn{1}{r}{\scriptsize \textcolor{darkgray}{Size: 7.3B}} \\
		\midrule
		\multirow{3}{*}{Base Methods} & Base Model & 0.00 & 0.00 & 100.0 & 100.0 & 0.00 & 0.00 & 100.0 & 100.0  \\
		& FT (vision block) & 39.58 & 0.98 & 100.0 & 3.96 & 0.63 & 0.00 & 100.0 & 5.13   \\
		& FT (last layer) & 39.57 & 0.58 & 72.01 & 16.42  & 2.75 &  0.00 & 35.52 & 9.28\\
            \midrule
		\multirow{4}{*}{Model Editing} & Knowledge Editor & \second{87.77} & \second{86.62}& 97.15 & \second{55.77} &  35.10 & 24.20 & 96.78 & \second{52.22}\\
		& In-Context Editing & 71.72 & 40.23 & 13.46 & 2.00 & \second{68.60} & \second{59.80} & 12.51 & 2.96 \\
		& SERAC & 87.20 & 84.60 & \first{100.0} & 0.33 & 40.20 & 36.60 & \first{100.0} & 0.97 \\
		& MEND & \first{95.51} & \first{95.27} & \second{98.73} & \first{71.33} & \first{87.10} & \first{84.10} & \second{98.34} & \first{59.53} \\
		\bottomrule

	\end{tabular}
        }
	%\hfill{}
	\caption{Main results on the {\ds}. 
 \textbf{T-Locality, M-Locality} refer to the textual and multimodal stability. 
 \textbf{T-Generality} represents textual generality. 
 \textbf{Reliability} denotes the accuracy of successful editing.} \label{tab:main-results}  
        
	%\vspace{-17pt}
\end{table*}
